Towards Zero-Waste Furniture Design

In traditional design, shapes are first conceived, and then fabricated. While this decoupling simplifies the design process, it can result in inefficient material usage, especially where off-cut pieces are hard to reuse. The designer, in absence of explicit feedback on material usage remains helpless to effectively adapt the design -- even though design variabilities exist. In this paper, we investigate {\em waste minimizing furniture design} wherein based on the current design, the user is presented with design variations that result in more effective usage of materials. Technically, we dynamically analyze material space layout to determine {\em which} parts to change and {\em how}, while maintaining original design intent specified in the form of design constraints. We evaluate the approach on simple and complex furniture design scenarios, and demonstrate effective material usage that is difficult, if not impossible, to achieve without computational support.

==> constraints.tex <==
\section{Furniture Design with Constraints \label{sec:constraints}}

% ---------------------------------------------------------------------------

During interaction with the system, either by the user or an algorithm optimizing
the design (see Sections~\ref{sec:material}), new design
points $\mbf{X}+\mbf{u}$ that violate the constraints are produced, with $\mbf{u}$
a vector of changes imposed. Typically, $\mbf{u}$ has only few non-zero entries,
e.g., the user or the optimizer increases a single plank length. Note that 
$\mbf{X}+\mbf{u}$ might violate either 
the design effectiveness constraints (i.e., $E\mbf{(X+u)} = {false}$), or the design constraints (i.e., $\mathbf{C} (\mbf{X}+\mbf{u}) \neq \mbf{s}$), or both.
We seek a correction vector $\mbf{d}$ such that $\mbf{X+u}+\mbf{d}$ is a valid design point
which preserves the changes applied by the system, that is $d_i = 0$ for all $i$ such that $u_i \neq 0$.

Our approach is based on two nested algorithms. The outer one solves
for design effectiveness constraints (see Section~\ref{sec:constraints:effectiveness}), while the inner one solves for design constraints (see Section~\ref{sec:constraints:design}). 

% Note that we generally assume that changes occur progressively, i.e.,  $||\mbf{d}||$ is small.


% ---------------------------------------------------------------------------

\subsection{Design Effectiveness Constraints Enforcement}
\label{sec:constraints:effectiveness}

We first describe how we resolve design effectiveness constraint violations.
These constraints are challenging to enforce as they cannot be simply expressed through
linear inequalities: detecting that a plank sags requires simulating the design under loads,
while preserving user specified inner volumes in the design requires detecting and
preventing collisions.

%\syl{To say somewhere before: the inner volumes are attached to planks and continuously move with the design.}

We observe that all the effectiveness constraints can be enforced by dynamically adding or removing
equality constraints. For instance, when a plank is about to sag
its length can be fixed to avoid lengthening it further. Similarly, when a plank
is about to enter an inner volume, a constraint can be inserted to maintain the
plank at the correct distance. A key difficulty is when and in which order
to insert the constraints. Note that a straightforward approach can quickly over-constrain the
problem, preventing to find a feasible solution.

Our scheme is inspired by collision detection in physics simulations, where all contacts
within a potentially large time step have to be found.
The intuition is to detect the first time a constraint violation occurs, while progressively applying
the change vector $\mbf{u}$. That is, we parameterize the problem with a variable $\alpha \in [0,1]$
and find the smallest value  $\alpha_1$ such that $E(\mbf{X} + \alpha_1 \mbf{u}) = {false}$. We
then add appropriate equality constraint to $\mbf{C,s}$ so that $E$ evaluates to true again. The algorithm
then recurses until reaching $\alpha = 1$, or encountering contradictory constraints (see Section~\ref{sec:constraints:infeasible}).
During this entire process we take care of enforcing design constraints while exploring along $\mbf{u}$.
All constraints added during the process are discarded upon termination.
The full algorithm is given in Algorithm~\ref{alg:Recusive}.

The function \texttt{CorrectForDesignConstraint} produces a correction vector recovering from design constraint
violations, and is described in Section~\ref{sec:constraints:design}.
The function \texttt{AddDynamicConstraints} considers the points just before and just after constraint
violation, and adds the equality constraints required to resolve the case. For instance, if a plank sags, it adds a constraint fixing
its length to be smaller by a margin to its current value in $\mbf{X}+l \cdot \mbf{u}$. If a plank
collides an inner volume of height $H$, it adds a constraint to keep the colliding plank at a distance
of $H$ of the plank supporting the inner volume. This is a very flexible approach allowing for a variety of
effectiveness constraints.

\begin{algorithm}[t!]
	\caption{\textsc{DynamicEffectivenessConstraints}}
	\label{alg:Recusive}
	\KwIn{Valid design $\mbf{X}$, vector of changes $\mbf{u}$, position $\alpha \leq 1$}
	\KwOut{A correction vector $\mbf{d}$ such that $\mathbf{C}(\mbf{X+u+d}) = \mbf{s}$ and $d_i = 0$ where $u_i \neq 0$ and $E(\mbf{X+u+d}) = true$}	
	$\mbf{d} \leftarrow $CorrectForConstraint$(\mbf{C},\mbf{s},\mbf{X},\mbf{u})$\;
	\If{$E(\mbf{X+u+d})$}{	
		\tcp{Found a solution, return}
		\Return $\mbf{d}$\;
    }
    \tcp{Search for first violation, bisection on $\alpha$}
	$\mbf{l} \leftarrow \alpha$\;	
	$\mbf{r} \leftarrow 1.0$\;		
	\While{$|l-r|>\epsilon$}
	{
		$\mbf{m} \leftarrow (\frac{l+r}{2}) \cdot \mbf{u}$\;
		$\mbf{d} \leftarrow $CorrectForDesignConstraint$(\mbf{C},\mbf{s},\mbf{X},\mbf{m})$\;
	    \If{$E(\mbf{X+m+d})$}{	
			${l} \leftarrow \frac{l+r}{2}$\;
		}\Else{
			${r} \leftarrow \frac{l+r}{2}$\;
		}
	}
	$\mbf{D,t} \leftarrow $AddDynamicConstraints$(\mbf{X}+l \cdot \mbf{u},\mbf{X}+r \cdot \mbf{u},\mbf{C},\mbf{s})$\;
	\If{$\mbf{D,t} = \mbf{C,s}$}{
		\tcp{No new constraint could be added: return best found so far}
		\Return $l \cdot \mbf{u}$\;
	}
\tcp{recurse}
\Return DynamicEffectivenessConstraints($\mbf{X},\mbf{u},l$)
\end{algorithm}

% ---------------------------------------------------------------------------

\subsection{Design Constraints Enforcement}
\label{sec:constraints:design}

We now describe how to recover a valid point while attempting to
preserve the latest changes made by the system. 
Let us consider a design point $\mbf{X+u}$ that violates some design constraints, i.e.,
$\mathbf{C} (\mbf{X+u}) \neq \mbf{s}$.
We seek a correction vector $\mbf{d}$ such that $\mathbf{C} (\mbf{X+u}+\mbf{d}) = \mbf{s}$
while preserving the changes applied by the system, that is $d_i = 0$ for all $i$ such that $u_i \neq 0$.
Note that we can ignore design effectiveness constraints ($E(\mbf{X})$) as they are taken
care of by the parent algorithm presented in Section~\ref{sec:constraints:effectiveness}.

In general, there are many possible solutions as the system is under-constrained. This ambiguity amounts to valid design choices. 
In addition to preserving the value of the variables being manipulated, it is also
desirable to limit the number of variables being adjusted by $\mbf{d}$,
so that variables seemingly not involved in the current user edits remain unchanged.
In other words, we seek a \textit{sparse} correction vector $\mbf{d}$. This
concentrates the changes on a few planks in the design, which results in a more
predictable interaction.


%In absence of other criteria, we could obtain a vector $\mbf{d}$
%by projecting $\mbf{X+u}$ onto the set of constraints. That is,
%solving for $\mbf{d}$ such that
%\[
%\begin{array}{ll}
%\mbf{d} & = \sum_i{ \lambda_i \mbf{c}_i }\\
%\mbf{d} \cdot \mbf{c}_i & = s_i - (\mbf{X+u}) \cdot \mbf{c}_i
%\end{array}
%\]
%\noindent where $\mbf{c}_i$ are the rows of $\mbf{C}$, and $\lambda_i$ are projection
%variables. The system has one variable per constraint ($\lambda_i$) and six per planks.
%It has a unique solution as long as the rows of $\mbf{C}$ are linearly independent,
%which we enforce when adding constraints by checking the rank of the system matrix.

% ---------------------------------------------------------------------------

\begin{algorithm}[t!]
	\caption{\textsc{CorrectForDesignConstraint}}
	\label{alg:solver}
	\KwIn{Linear system of constraints $\mathbf{C},\mbf{s}$,
		  a valid design point $\mbf{X}$,
		  a vector of changes $\mbf{u}$}
	\KwOut{A correction vector $\mbf{d}$ such that $\mathbf{C}(\mbf{X+u+d}) = \mbf{s}$ and $d_i = 0$ where $u_i \neq 0$}	
	$\Lambda \leftarrow \emptyset$\;
	$\mbf{d} = \mbf{0}$\;
	$\mbf{r} = \mathbf{C}(\mbf{X+u}+\mbf{d}) - \mbf{s}$\;
	\While{true}{ \label{line:loop-begin}
	    $\mathcal{N} \leftarrow$ \{variables from non-satisfied constraints ($r_i \neq 0$)\}\;
		$\mathcal{T} \leftarrow \mathcal{N} \setminus (\Lambda \cup \lbrace i | u_i \neq 0 \rbrace)$\;
		\If{$\mathcal{T} = \emptyset$}{
			\tcp{Cannot solve: backtrack}
			Fail\;
		}
		\ForEach{$v_i \in \mathcal{T}$}
		{
			\tcp{Estimate how variable will move}
			\tcp{Variable $v_i$ corresponds to column $c_i$ in $\mbf{C}$}
			$m = - {\mbf{c}_i^\intercal \mbf{r}}/{\mbf{c}_i^\intercal \mbf{c}_i}$\;
			$score(v_i)$ = 0\;
			\If{$v_i \in \{l^x,l^y,l^z\}$ {and $m$ violates min length on $v_i$}}
			{
				\tcp{Preserve min edge length constraint}
			    $score(v_i)$ = $- \infty$\;
			}
			\ElseIf{$v_i \in \{l^x,l^y,l^z\}$}
			{
				\tcp{Penalize change in length}
				$score(v_i)$ = $- |m|$\;			
			}
			\If{$score(v_i) > score(b)$} {
				$b \gets v_i$\;
			}
		}
		$\Lambda = \Lambda \cup \{b\}$\;
		$\mbf{d} = $ SolvePartialCorrectionVector($\Lambda$,$\mathbf{C}$,s,$\mbf{X+u}$)\;
		$\mbf{r} = \mathbf{C}(\mbf{X+u}+\mbf{d}) - \mbf{s}$\;
		\If{ $||\mbf{r}|| < \epsilon$ }{
			\Return $\mbf{d}$\;
		}
	}
\end{algorithm}


% ---------------------------------------------------------------------------

Our approach is inspired by the works of
Bokeloh et al.~\shortcite{Bokeloh:2012:AMP} and Habbecke and Kobbelt~\shortcite{habbecke.12.cgf}.
The key idea is to solve for $d$ using only a subset of the variables in $\mbf{X}$.
Let us denote canonical basis vectors $\mathbf{B_k} = (0,...,1,...0)$
with $k-1$ leading zeros, and $\Lambda$ a set of variable indices that are allowed
to change.
%
Then, we can express the correction vector $\mbf{d}$ as:
$
\mbf{d}_\Lambda = \sum_{k\in\Lambda}{d_k \mathbf{B_k}}.
$
%
Hence, the system takes the form:
\[
\begin{array}{ll}
\text{for all }k \in \Lambda\\[2mm]
d_k & = \sum_i{ \lambda_i c_{ik} }\\[2mm]
\sum_k{d_k \cdot c_{ik}} & = s_i - \mbf{p} \cdot \mbf{c}_i
\end{array}
\]
The system is often under-determined after removing variables. We solve it
by QR decomposition and computing the pseudo-inverse of the system matrix.
Given a set $\Lambda$, solving for $\mbf{d}_\Lambda$ results in a residual
$\varepsilon(\mbf{d}_\Lambda) = \| \mbf{C} (\mbf{X}+\mbf{d}_\Lambda) - s \|$. We accept solutions when $\|\varepsilon(\mbf{d}_\Lambda)\| < \epsilon$ with $\epsilon$ a small constant
($10^{-9}$ mm in our implementation).
We use the Eigen library~\shortcite{eigenweb} for solving all linear systems.


%An alternative formulation consists in
%computing the nullspace of the constraint matrix $\mbf{C}$ and project into a subset
%of the basis vectors~\cite{habbecke.12.cgf}.

Our approach is inspired by Orthogonal Basis Pursuit~\cite{Chen:2001:ADB},
which greedily selects the next variable based on the residual, until
it becomes small enough. We follow a similar greedy strategy using the following criteria to prioritize:
\begin{enumerate}
\item Change as few variables as possible, which is minimizing $|\Lambda|$.
\item Avoid changes that would violate the minimal plank lengths, which is
where $l^a_i + d_i < M^a_i$.
\item Avoid changes to the plank lengths, and favor changes in plank positions
instead. Indeed, length variables are generally more important than the
positional variables: most furniture designs are fully connected, and hence
plank lengths are enough to describe the full design up to a translational
degree of freedom.
\end{enumerate}

The algorithm for variable selection is given in Algorithm~\ref{alg:solver}.
Function {\tt SolvePartialCorrectionVector} implements the projection using
a subset of the variables. We initialize
$\Lambda$ with the indices of the variables of newly added planks, so that they are changed
first and do not impact the current design. Thus, $\Lambda$ will never contain indices such that $u_i \neq 0$, and thereby
protect the changes made by $\mbf{u}$.

% ---------------------------------------------------------------------------

\subsection{Failure cases}
\label{sec:constraints:infeasible}

The system can fail to solve (see Algorithm~\ref{alg:solver}, line 8 and  Algorithm~\ref{alg:Recusive}, line 15).
This typically happens of the user makes contradictory changes (e.g., attempting to modify the length of
a planks having a fixed length constraint), or when the environmental constraints cascade into a similar
contradiction.

In such cases, the user can choose to violate the constraints ({\em override mode}, see Section~\ref{sec:overview}). 
The system then provides a visual feedback of the constraints in error. Alternately, the user may also choose to accept the partial solution
proposed by the system ({\em flush mode}). When the system is calling the solver,
as is the case for the suggestion system described in Section~\ref{sec:pack:suggest}, the flush mode is always used.


==> fem.tex <==
%
% Figure to show voxels overlaid on planks, density in elements will change
%

\section*{Appendix: Detecting Plank Sagging} % of Furniture}

This appendix discusses our sagging detection, which has two main
steps: first, computation of a displacement field by the finite element
method (FEM); second, analysis of the displacement field to detect sagging.

\mypara{Computing displacement field}
We assume a homogeneous material and assume that connectors are
perfectly glued.  Note that the displacement field could be computed with any available simulation
%
%\begin{wrapfigure}{r}{0.5\columnwidth}
%\vspace{-10pt}
%  \begin{center}
%    \includegraphics[width=0.5\columnwidth]{./figures/compliance/element_density.pdf}  
%  \end{center}
%  \vspace{-10pt}
%\end{wrapfigure} 
%
software for structural analysis. In our implementation, to achieve fast feedback and avoid
(re)meshing the design, we decouple the simulation elements from the
exact location of the planks.
We rely on a uniform grid of cubic (hexahedral) elements, where each cubic
element receives a relative density value $\rho_e \in [0,1]$. The elements have a fixed
size of 10 mm, planks have a typical thickness of 3 mm. When a plank intersects an element,
the element receives a density which corresponds to the fraction of the intersected cube volume.

The stiffness matrix of an element is given
by $\mbf{K}_e(\rho_e) := \rho_e \mbf{K}_{c}$, where $\mbf{K}_{c}$
represents the stiffness matrix of a unit cubic element. Note that the stiffness
matrix is a function of the element density. We obtain 
$\mbf{K}_{c}$ from the elastic material parameters using standard
finite element integration over a cube. The design is assumed to be fixed to the ground (at its points of
attachment), while all the other non-ground touching nodes are assumed to be free.

Using the FEM, we compute a vector of displacements $\mathbf{u}$ as
the solution of the linear system $\mathbf{K}(\boldsymbol{\rho}) \mathbf{u} = \mathbf{f}$, where
$\boldsymbol{\rho}$ is the vector of all element densities, $\mathbf{K}(\boldsymbol{\rho})$ is the
global stiffness matrix of the design, assembled from the element matrices, and $\mathbf{f}$ encodes
the forces applied to the system.


\mypara{Detecting sagging}
We note that sagging is a relative notion, i.e., a plank might be rigidly displaced due to other planks sagging in the design.
We analyze sagging by considering several sample points on each plank surface (a $32 \times 32$ uniform sampling). We obtain the displacement of each sample using tri-linearly interpolation from the displacements of the grid nodes computed with the FEM. 

For a given axis, we define sagging as the deflection between the sample point and a straight line from the plank edges passing 
\begin{wrapfigure}[4]{r}{3cm}
	\vspace*{-4mm}
	\hspace*{-8mm}
	\includegraphics[width=3.5cm]{figures/sagdetect/sagdetect.png}
\end{wrapfigure}
above the sample. This is illustrated in the figure inset; the sample point is in black, the straight line from edges in orange.
For each sample we compute the difference between the displacement at the sample point and the displacement interpolated linearly from the edges. The difference is shown in red in the figure inset. If the difference is above a threshold (e.g., 0.2 mm) the plank is tagged as sagging. 

